Irregular Repetition Slotted ALOHA Over the Binary Adder Channel

We propose an irregular repetition slotted ALOHA (IRSA) based random-access protocol for the binary adder channel (BAC). The BAC captures important physical-layer concepts, such as packet generation, per-slot decoding, and information rate, which are neglected in the commonly considered collision channel model. We divide a frame into slots and let users generate a packet, to be transmitted over a slot, from a given codebook. In a state-of-the-art scheme proposed by Paolini et al. (2022), the codebook is constructed as the parity-check matrix of a BCH code. Here, we construct the codebook from independent and identically distributed binary symbols to obtain a random-coding achievability bound. Our per-slot decoder progressively discards incompatible codewords from a list of candidate codewords, and can be improved by shrinking this list across iterations. In a regime of practical interests, our scheme can resolve more colliding users in a slot and thus achieves a higher average sum rate than the scheme in Paolini et al. (2022).

==> fig/PLR_fixedPayload.tex <==
\begin{tikzpicture}[scale=.85]
				\begin{axis}[%
					width=1.75in,
					height=2in,
					scale only axis,
					unbounded coords=jump,
					xmin=0,
					xmax=3,
					%					xtick={1,2,3,4,5,6,7},
					xlabel style={font=\color{white!15!black},yshift=4pt},
					xlabel={Channel load $G = \mu K/N$},
					ymin=1e-6,
					ymax=1,
					ymode=log,
					yminorticks=true,
					ytick={1e0,1e-2,1e-4,1e-6},
					ylabel style={font=\color{white!15!black},yshift=-18pt},
					ylabel={PLR},
					axis background/.style={fill=white},
					title style={font=\bfseries},
					%title={$\Lambda^{(1)}(x) = \Lambda^{(2)}(x) = x$},
					xmajorgrids,
					ymajorgrids,
					%yminorgrids,
					legend style={at={(.01,0.99)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
					]
					
					\addplot [line width = 1.5,color=black]
					table[row sep=crcr]{%
						0.100000000000000   0.000015402780972 \\
						0.200000000000000   0.000031623282065 \\
						0.300000000000000   0.000050566361583 \\
						0.400000000000000   0.000070063033355 \\
						0.500000000000000   0.000123815789061 \\
						0.600000000000000   0.004347571068982 \\
						0.700000000000000   0.094316670097961 \\
						0.800000000000000   0.388386821381553 \\
						0.900000000000000   0.646566411977005 \\
						1.000000000000000   0.779028815859255 \\
						1.100000000000000   0.852667135251769 \\
						1.200000000000000   0.897832260035415 \\
						1.300000000000000   0.928297108775040 \\
						1.400000000000000   0.948970818721066 \\
						1.500000000000000   0.963218067102386 \\
						1.600000000000000   0.973399445066187 \\
						1.700000000000000   0.980644758392464 \\
						1.800000000000000   0.985861329242355 \\
						1.900000000000000   0.989651435615898 \\
						2.000000000000000   0.992365681393433 \\
						2.100000000000000   0.994390742159594 \\
						2.200000000000000   0.995856420155059 \\
						2.300000000000000   0.996951663919501 \\
						2.400000000000000   0.997748039944295 \\
						2.500000000000000   0.998339752748028 \\
						2.600000000000000   0.998771399179175 \\
						2.700000000000000   0.999093791488377 \\
						2.800000000000000   0.999326949180869 \\
						2.900000000000000   0.999504464823820 \\
						3.000000000000000   0.999635746976700 \\
%						0.100000000000000   0.000016146772260 \\
%						0.200000000000000   0.000030252530624 \\ 
%						0.300000000000000   0.000049332999513 \\
%						0.400000000000000   0.000068560000988 \\
%						0.500000000000000   0.000120402043833 \\
%						0.600000000000000   0.004494993280178 \\
%						0.700000000000000   0.092970758404691 \\
%						0.800000000000000   0.388757240784598 \\
%						0.900000000000000   0.646021254316389 \\
%						1.000000000000000   0.779071259608220 \\
%						1.100000000000000   0.852591368462467 \\
%						1.200000000000000   0.898131345231077 \\
%						1.300000000000000   0.928343794302411 \\
%						1.400000000000000   0.948927855780838 \\
%						1.500000000000000   0.963281017836613 \\
%						1.600000000000000   0.973319904054131 \\
%						1.700000000000000   0.980664243570112 \\
%						1.800000000000000   0.985832580797690 \\
%						1.900000000000000   0.989641200219127 \\
%						2.000000000000000   0.992368614906068 \\
					};
					\node[rotate=83,color=black] at (axis cs:.46,5e-3) () {Original IRSA};
					%				\addlegendentry{\small PD-SPR};
					
					\addplot [line width = 1.5,color=red]
					table[row sep=crcr]{%
						0.100000000000000                   0 \\
						0.200000000000000   0.000000150010156 \\
						0.300000000000000   0.000000399982107 \\
%						0.400000000000000   0.000001087322794 \\
						0.500000000000000   0.000000950039389 \\
						0.600000000000000   0.000001441498399 \\
						0.700000000000000   0.000001578502805 \\
						0.800000000000000   0.000002018846690 \\
						0.900000000000000   0.000003460438421 \\
						1.000000000000000   0.000077086572016 \\
						1.100000000000000   0.001068949484940 \\
						1.200000000000000   0.034634915269793 \\
						1.300000000000000   0.214917472693548 \\
						1.400000000000000   0.484889509641980 \\
						1.500000000000000   0.679821417149923 \\
						1.600000000000000   0.794484131397204 \\
						1.700000000000000   0.846335819839215 \\
						1.800000000000000   0.895772387664861 \\
						1.900000000000000   0.927612507306438 \\
						2.000000000000000   0.950160786165643 \\
						2.100000000000000   0.964796645266840 \\
						2.200000000000000   0.975854657053134 \\
						2.300000000000000   0.983208868383264 \\
						2.400000000000000   0.988498433044070 \\
						2.500000000000000   0.992098012889420 \\
						2.600000000000000   0.992904427170523 \\
						2.700000000000000   0.995068350380622 \\
						2.800000000000000   0.996571654753445 \\
						2.900000000000000   0.997595803797875 \\
						3.000000000000000   0.998353875865011 \\
%						0.100000000000000   0.000000090002226 \\
%						0.200000000000000   0.000000712473168 \\
%						0.300000000000000   0.000001088325508 \\
%						0.400000000000000   0.000001551285777 \\
%						0.500000000000000   0.000002526939509 \\
%						0.600000000000000   0.000003101504027 \\
%						0.700000000000000   0.000004357696543 \\
%						0.800000000000000   0.000007268299744 \\
%						0.900000000000000   0.000009800313348 \\
%						1.000000000000000   0.000276184196740 \\
%						1.100000000000000   0.017710888548016 \\
%						1.200000000000000   0.160165870929698 \\
%						1.300000000000000   0.269017211634868 \\
%						1.400000000000000   0.528263486967703 \\
%						1.500000000000000   0.701770133893457 \\
%						1.600000000000000   0.807079610561446 \\
%						1.700000000000000   0.873588656670417 \\
%						1.800000000000000   0.916443689373772 \\
%						1.900000000000000   0.944880085576234 \\
%						2.000000000000000   0.963734130528788 \\
					};
					\node[rotate=82.5,color=red] at (axis cs:.98,2e-3) () {Our scheme, ED-MPR};
					%					\addlegendentry{\small Our original scheme};
					
					\addplot [line width = 1.5,color=OliveGreen]
					table[row sep=crcr]{%
%%						1 1.4286e-05 \\
%						1.2 8.1633e-08 \\
%%						1.4 1.4520e-05 \\
%						1.5 0.008148005621262 \\
%%						1.6 2.4491e-05 \\
%						1.8 0.0814 \\
%						1.9 0.5414 \\
%						2 0.6390 \\
%						2.1 0.7132 \\
                        1.2 8.097165991902799e-08 \\ 
						1.4 1.5707e-05 \\
						1.500000000000000   0.003860666496792 \\
						1.600000000000000   0.070595978907076 \\
						1.700000000000000   0.240205798532610 \\
						1.800000000000000   0.588162955673359 \\
						1.900000000000000   0.792790424044599 \\
						2.000000000000000   0.923112724436456 \\
						2.100000000000000   0.951344165283176 \\
						2.200000000000000   0.961705304899277 \\
						2.300000000000000   0.973355131979843 \\
						2.400000000000000   0.988498433044070 \\
						2.500000000000000   0.992098012889420 \\
						2.600000000000000   0.992904427170523 \\
						2.700000000000000   0.995068350380622 \\
						2.800000000000000   0.996571654753445 \\
						2.900000000000000   0.997595803797875 \\
						3.000000000000000   0.998353875865011 \\
					};
					\node[rotate=84,color=OliveGreen] at (axis cs:1.62,1e-3) () {Our scheme, ED-FG};
					%					\addlegendentry{\small Our improved scheme};
					
					%					\node[] at (axis cs:0.4,0.02) () {\large $\delta = 0.9$};
					
					% \addplot [line width = 1.5,dotted,color=blue]
					% table[row sep=crcr]{%
						% 	1.675459656815819 1e-6    \\ 
						% 	1.675459656815819 1 \\ 
						% };
					
					% \addplot [line width = 1.5,dotted,color=red]
					% table[row sep=crcr]{%
						% 	2.574702557012240 1e-6    \\ 
						% 	2.574702557012240 1 \\ 
						% };
				\end{axis}
			\end{tikzpicture}

==> fig/PLR_vs_g.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[scale=.75]
	
	\begin{axis}[%
		width=4.5in,
		height=3.5in,
		%at={(0.545in,0.436in)},
		scale only axis,
		unbounded coords=jump,
		xmin=0,
		xmax=2,
		xlabel style={font=\color{white!15!black},yshift=4pt},
		xlabel={Channel load $G$},
		ymode=log,
		ymin=1e-04,
		ymax=1,
		yminorticks=true,
		ylabel style={font=\color{white!15!black},yshift=-4pt},
		ylabel={Packet loss rate},
		axis background/.style={fill=white},
		title style={font=\bfseries},
		%title={$\Lambda^{(1)}(x) = \Lambda^{(2)}(x) = x$},
		xmajorgrids,
		ymajorgrids,
		%yminorgrids,
		legend style={at={(.99,0.02)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
		]
		
		\addplot [line width = 1,color=blue]
		table[row sep=crcr]{%
			0.1 0.0044427\\
			0.2 0.0097086\\
			0.3 0.020755\\
			0.4 0.041889\\
			0.5 0.084128\\
			0.6 0.1572\\
			0.7 0.26588\\
			0.8 0.39517\\
			0.9 0.52789\\
			1 0.63821\\
			1.1 0.72422\\
			1.2 0.79214\\
			1.3 0.83879\\
			1.4 0.87604\\
			1.5 0.90312\\
			1.6 0.92403\\
			1.7 0.9401\\
			1.8 0.95399\\
			1.9 0.96332\\
			2 0.97101\\
		};
		\addlegendentry{\small Peeling decoder, SPR};
		
		\addplot [line width = 1,color=red]
		table[row sep=crcr]{%
			0.1 0.0015737\\
			0.2 0.0032361\\
			0.3 0.0048873\\
			0.4 0.0066392\\
			0.5 0.0093091\\
			0.6 0.014203\\
			0.7 0.020153\\
			0.8 0.033037\\
			0.9 0.054583\\
			1 0.093769\\
			1.1 0.15522\\
			1.2 0.23577\\
			1.3 0.34443\\
			1.4 0.45322\\
			1.5 0.5638\\
			1.6 0.66064\\
			1.7 0.74281\\
			1.8 0.80197\\
			1.9 0.85063\\
			2 0.88421\\
		};
		\addlegendentry{\small Peeling decoder, MPR};
		
		\addplot [line width = 1,color=cyan]
		table[row sep=crcr]{%
			0.1 0.0010\\
			0.2 0.0023\\
			0.3 0.0020\\
			0.4 0.0032\\
			0.5 0.0036\\
			0.6 0.0060\\
			0.7 0.0077\\
			0.8 0.0081\\
			0.9 0.0090\\
			1 0.0110\\
			1.1 0.0111\\
			1.2 0.0123\\
			1.3 0.0171\\
			1.4 0.0299\\
			1.5 0.0465\\
			1.6 0.1112\\
			1.7 0.1628\\
			1.8 0.2622\\
			1.9 0.3572\\
			2 0.4683\\
		};
		\addlegendentry{\small List-passing decoder};
		
		\addplot [line width = 1,color=magenta]
		table[row sep=crcr]{%
			0.1 0.0014972\\
			0.2 0.0018734\\
			0.3 0.0039715\\
			0.4 0.0048983\\
			0.5 0.0094278\\
			0.6 0.010426\\
			0.7 0.015235\\
			0.8 0.016407\\
			0.9 0.021462\\
			1 0.02368\\
			1.1 0.028882\\
			1.2 0.02936\\
			1.3 0.036429\\
			1.4 0.040588\\
			1.5 0.047534\\
			1.6 0.05407\\
			1.7 0.06676\\
			1.8 0.076279\\
		};
		\addlegendentry{\small HIC decoder, nontrinsic};
		
		\addplot [line width = 1,color=magenta, dashed]
		table[row sep=crcr]{%
			0.1 0.64883\\
			0.2 0.74892\\
			0.3 0.77964\\
			0.4 0.79785\\
			0.5 0.80355\\
			0.6 0.80927\\
			0.7 0.81712\\
		};
		\addlegendentry{\small HIC decoder, extrinsic};
		
	\end{axis}
	
\end{tikzpicture}%

==> fig/PLR_vs_g_thres.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[scale=.75]
	
	\begin{axis}[%
		width=4.5in,
		height=3.5in,
		%at={(0.545in,0.436in)},
		scale only axis,
		unbounded coords=jump,
		xmin=0,
		xmax=2,
		xlabel style={font=\color{white!15!black},yshift=4pt},
		xlabel={Channel load $G$},
		ymode=log,
		ymin=1e-03,
		ymax=1,
		yminorticks=true,
		ylabel style={font=\color{white!15!black},yshift=-4pt},
		ylabel={Packet loss rate},
		axis background/.style={fill=white},
		title style={font=\bfseries},
		%title={$\Lambda^{(1)}(x) = \Lambda^{(2)}(x) = x$},
		xmajorgrids,
		ymajorgrids,
		%yminorgrids,
		legend style={at={(.1,0.02)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
		]
		
		\addplot [line width = 1,color=blue]
		table[row sep=crcr]{%
			0.1 0.0039739\\
			0.2 0.0044909\\
			0.3 0.0091688\\
			0.4 0.012005\\
			0.5 0.014111\\
			0.6 0.017944\\
			0.7 0.021371\\
			0.8 0.024952\\
			0.9 0.039492\\
			1 0.050414\\
			1.1 0.072237\\
			1.2 0.10855\\
			1.3 0.14938\\
			1.4 0.19819\\
			1.5 0.2425\\
			1.6 0.29092\\
			1.7 0.34895\\
		};
		\addlegendentry{\small Simulation, $n_0 = 10$};
		
		\addplot [line width = 1,color=blue, dashed]
		table[row sep=crcr]{%
			1.4226 1e-4 \\
			1.4226 1 \\
		};
		\addlegendentry{\small Decoding threshold, $n_0 = 10$};
		
		\addplot [line width = 1,color=magenta]
		table[row sep=crcr]{%
			0.1 0.0015\\
			0.2 0.0043\\
			0.3 0.0077\\
			0.4 0.0110\\
			0.5 0.0128\\
			0.6 0.0176\\
			0.7 0.0198\\
			0.8 0.0219\\
			0.9 0.0282\\
			1 0.0408\\
			1.1 0.0528\\
			1.2 0.0715\\
			1.3 0.0957\\
			1.4 0.1326\\
1.5000    0.1645 ==
%			1.6 0.29092\\
%			1.7 0.34895\\
		};
		\addlegendentry{\small Simulation, $n_0 = 11$};
		
		\addplot [line width = 1,color=magenta, dashed]
		table[row sep=crcr]{%
			1.7558 1e-4 \\
			1.7558 1 \\
		};
		\addlegendentry{\small Decoding threshold, $n_0 = 11$};
	\end{axis}
	
\end{tikzpicture}%

==> fig/defs.tex <==
\usepackage{bm}
\usepackage{upgreek}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{xspace}

\safemath{\mi}{I}
\safemath{\difent}{\mathrm{h}}		%differential entropy
\safemath{\NonnegReal}{\mathbb{R}^{+}}


\safemath{\indist}{\cdfP} %input distribution
\safemath{\outdist}{\cdfQ} %output distribution
\safemath{\inpdf}{\pdfp} %input pdf
\safemath{\outpdf}{\pdfq} %output pdf
\safemath{\testdist}{\cdfP} %the distribution of test P_{Z|W}

%\safemath{\tr}[#1]{\mathrm{tr}\left\lbrace #1  \right\rbrace}

\safemath{\powallocvec}{\vecv}
\safemath{\powalloc}{v}
\safemath{\encoder}{f} % the encoder of the code
\safemath{\decoder}{g} % the decoder of the code
\safemath{\msg}{J} % the message
\safemath{\csir}{\mathrm{r}}
\safemath{\csit}{\mathrm{t}}
\safemath{\csi}{\mathrm{csi}}
\safemath{\csirt}{\mathrm{rt}}
\safemath{\Rcsirt}{R_{\csirt}} %rate with CSIT
\safemath{\Rcsir}{R_{\csir}}
\safemath{\Rcsit}{R_{\csit}}
\safemath{\cohblock}{T}
\safemath{\blocklength}{n}
\safemath{\selbranches}{L}


\safemath{\Rnocsit}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rnocsi}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rgeneral}{R_{\mathrm{no,rt}}} %rate with general CSI condition
\safemath{\equalR}{R_{\mathrm{e}}}

\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl[\genfrac..{0pt}{}{#3}{#4};#5\biggr]%
        \endgroup
}

%------------------------------------
%		JOHAN
%------------------------------------
\safemath{\Rmax}{R^*(n,\epsilon)} %rate without CSIT
\safemath{\codewords}{K}
\safemath{\Rub}{\bar{R}(n,\epsilon)}
\safemath{\Rlb}{\underline{R}(n,\epsilon)}
\safemath{\rk}{\kappa}
\safemath{\rlos}{\bar{\matH}}
\safemath{\rnlos}{\tilde{\randmatH}}

\safemath{\randtemp}{K}

\safemath{\Vnocsit}{V_{\error}^{\mathrm{no}}}
\safemath{\Vcsit}{V_{\error}^{\mathrm{rt}}}

\safemath{\cadist}{F_C} %capacity distribution
\safemath{\cdistno}{F_{0}}
\safemath{\cdistcsit}{F_{1}}


\safemath{\deF}{d_0} %the derivative of F_C(\xi) %\left.\frac{d\cadist(\argpn)}{d\argpn}\right|_{\argpn=C_\error}

\safemath{\bl}{n} %block length
\safemath{\blt}{\tilde{\bl}}
\safemath{\error}{\epsilon} %prob of error
\safemath{\NumCode}{M}
\safemath{\RXant}{r}
%\safemath{\rxant}{r}
%\safemath{\txant}{t}
\safemath{\txantop}{t^{\ast}}
\safemath{\minant}{m}
\safemath{\minantop}{\minant^\ast}
\safemath{\snr}{\rho}
\safemath{\const}{k}
\safemath{\inset}{\setF} %the input power set
\safemath{\spanm}{\mathrm{span}}
\safemath{\ubb}{b_{0}}%upper bound of b_1,...,b_{r} of the matrix I+ H^H U H.

%%%%%%%%%%%MIMO%%%%%%%%%%%%%%%%%%%%
\safemath{\covmat}{\matU}
\safemath{\covmatY}{\matV}
\safemath{\randcmY}{\randmatV}

\safemath{\insetMIMO}{\setF_{\txant,\bl}}
\safemath{\insetcov}{\setU_{\txant}}
%\safemath{\condcov}{\matQ\succeq\mathbf{0},\tr(\matQ)\leq\snr}
\safemath{\condcov}{\matQ\in\insetcov}

\safemath{\BoundFU}{k_{\delta}}

\safemath{\argpn}{\xi} % the argument in the probability p(R)

\safemath{\angletest}{Z} %the angle test used in achievability part

\safemath{\Cnocsit}{C_{\epsilon}^{(0)}}
\safemath{\Ccsit}{C_{\epsilon}^{(1)}}

\safemath{\errorach}{P_\mathrm{e}} %the error in intuition part



\newcommand{\given}{\,\vert\,}				% conditioning
\newcommand{\ggiven}{\,\Vert\,}
\safemath{\define}{\triangleq}			% definition
%\safemath{\fnorm}{\mathrm{F}}

\safemath{\altbl}{\tilde{\bl}}
\safemath{\constL}{k_{\mathrm{L}}}
\safemath{\constU}{k_{\mathrm{U}}}
\safemath{\funcL}{\tilde{q}}
\safemath{\funcU}{q}
\safemath{\ConstThm}{k_0}
%%%%%%%%%%%%%%%%used in the intuition part %%%%%%%%%%%%%
\safemath{\randrevec}{\randvecy}
\safemath{\revec}{\vecy}
\safemath{\trcwd}{\vecx}
\safemath{\randtrcwd}{\randvecx}
\safemath{\randnoisevec}{\randvecw}
\safemath{\transmitcwd}{\vecx_1} %the transmitted codeword in achievability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%used in the appendix of proving gamma=C_error + O(1/\bl) %%%%%%%%%%%%%
\safemath{\pickcwdnoch}{\vecx_0} %the chosen codeword x=[P,P,...,P]
\safemath{\pickcwd}{\vecx_0} %the chosen codeword x=[P,P,...,P]

\safemath{\inseqrand}{\randvecx}
\safemath{\inseq}{\vecx}

\safemath{\outseq}{\matY}
\safemath{\outseqrand}{\randmatY}

%used in the appendix of the proof of achievability
\safemath{\altT}{\widetilde{T}}
\safemath{\altU}{\widetilde{U}}
\safemath{\altmean}{\tilde{\mu}}
\safemath{\altvar}{\tilde{\sigma}}
\safemath{\altf}{\funcL}
\safemath{\altg}{\tilde{g}}
\safemath{\altgamma}{\tilde{\gamma}}
\safemath{\altdelta}{\tilde{\delta}}
\safemath{\altk}{\tilde{k}}
\safemath{\altconst}{\altk}
\safemath{\altbmLambda}{\widetilde{\bm{\Lambda}}}
\safemath{\constant}{\tilde{k}}
\safemath{\ntot}{n\sub{tot}}


==> fig/glossary.tex <==
\newglossaryentry{wlog}
{
	name={w.l.o.g.},
	description={without loss of generality},
	first={\glsentrydesc{wlog} (\glsentrytext{wlog})}
}


\newglossaryentry{sic}
{
	name={SIC},
	description={successive interference cancellation},
	first={\glsentrydesc{sic} (\glsentrytext{sic})}
}

\newglossaryentry{plr}
{
	name={PLR},
	description={packet loss rate},
	first={\glsentrydesc{plr} (\glsentrytext{plr})}
}

\newglossaryentry{pupe}
{
	name={PUPE},
	description={per-user probability of error},
	first={\glsentrydesc{pupe} (\glsentrytext{pupe})}
}

\newglossaryentry{pmf}
{
	name={PMF},
	description={probability mass function},
	first={\glsentrydesc{pmf} (\glsentrytext{pmf})}
}

\newglossaryentry{bpsk}
{
	name={BPSK},
	description={binary phase shift keying},
	first={\glsentrydesc{bpsk} (\glsentrytext{bpsk})}
}

\newglossaryentry{bac}
{
	name={BAC},
	description={binary adder channel},
	first={\glsentrydesc{bac} (\glsentrytext{bac})}
}

\newglossaryentry{mac}
{
  name={MAC},
  description={multiple-access channel},
  first={\glsentrydesc{mac} (\glsentrytext{mac})}
}

\newglossaryentry{simo}
{
	name={SIMO},
	description={single-input multiple-output},
	first={\glsentrydesc{simo} (\glsentrytext{simo})}
}

\newglossaryentry{mmse}
{
  name={MMSE},
  description={minimum mean-square error},
  first={\glsentrydesc{mmse} (\glsentrytext{mmse})}
}

\newglossaryentry{na}
{
  name={NA},
  description={normal approximation},
  first={\glsentrydesc{na} (\glsentrytext{na})},
  plural={NAs},
  descriptionplural={normal approximations},
  firstplural={\glsentrydescplural{na} (\glsentryplural{na})}
}

\newglossaryentry{zf}
{
  name={ZF},
  description={zero-forcing},
  first={\glsentrydesc{zf} (\glsentrytext{zf})}
}

\newglossaryentry{rzf}
{
  name={RZF},
  description={regularized zero-forcing},
  first={\glsentrydesc{rzf} (\glsentrytext{rzf})}
}

\newglossaryentry{sir}
{
  name={SIR},
  description={signal-to-interference ratio},
  first={\glsentrydesc{sir} (\glsentrytext{sir})}
}

\newglossaryentry{mse}
{
  name={MSE},
  description={mean-square error},
  first={\glsentrydesc{mse} (\glsentrytext{mse})}
}
\newglossaryentry{mmmse}
{
  name={M-MMSE},
  description={multicell MMSE},
  first={\glsentrydesc{mmmse} (\glsentrytext{mmmse})}
}

\newglossaryentry{ls}
{
  name={LS},
  description={least-squares},
  first={\glsentrydesc{ls} (\glsentrytext{ls})}
}

\newglossaryentry{mr}
{
  name={MR},
  description={maximum ratio},
  first={\glsentrydesc{mr} (\glsentrytext{mr})}
}

\newglossaryentry{ue}
{
  name={UE},
  description={user equipment},
  first={\glsentrydesc{ue} (\glsentrytext{ue})},
  plural={UEs},
  descriptionplural={user equipments},
  firstplural={\glsentrydescplural{ue} (\glsentryplural{ue})}
}

\newglossaryentry{ap}
{
  name={AP},
  description={access point},
  first={\glsentrydesc{ap} (\glsentrytext{ap})},
  plural={APs},
  descriptionplural={access points},
  firstplural={\glsentrydescplural{ap} (\glsentryplural{ap})}
}

\newglossaryentry{cpu}
{
  name={CPU},
  description={central processing unit},
  first={\glsentrydesc{cpu} (\glsentrytext{cpu})},
  plural={CPUs},
  descriptionplural={central processing units},
  firstplural={\glsentrydescplural{cpu} (\glsentryplural{cpu})}
}

\newglossaryentry{bs}
{
  name={BS},
  description={base station},
  first={\glsentrydesc{bs} (\glsentrytext{bs})},
  plural={BSs},
  descriptionplural={base stations},
  firstplural={\glsentrydescplural{bs} (\glsentryplural{bs})}
}


\newglossaryentry{ostbc}
{
  name={OSTBC},
  description={orthogonal space-time block code},
  first={\glsentrydesc{ostbc} (\glsentrytext{ostbc})},
  plural={OSTBCs},
  descriptionplural={orthogonal space-time block codes},
  firstplural={\glsentrydescplural{ostbc} (\glsentryplural{ostbc})}
}

\newglossaryentry{biawgn}
{
  name={bi-AWGN},
  description={binary-input additive white Gaussian noise},
  first={\glsentrydesc{biawgn} (\glsentrytext{biawgn})}
}

\newglossaryentry{flnf}
{
  name={FLNF},
  description={fixed-length no-feedback},
  first={\glsentrydesc{flnf} (\glsentrytext{flnf})}
}

\newglossaryentry{crc}
{
  name={CRC},
  description={cyclic redundancy check},
  first={\glsentrydesc{crc} (\glsentrytext{crc})}
}

\newglossaryentry{bsc}
{
  name={BSC},
  description={binary symmetric channel},
  first={\glsentrydesc{bsc} (\glsentrytext{bsc})}
  plural={BSCs},
  descriptionplural={binary symmetric channels},
  firstplural={\glsentrydescplural{bsc} (\glsentryplural{bsc})}
}


\newglossaryentry{bec}
{
  name={BEC},
  description={binary-erasure channel},
  first={\glsentrydesc{bec} (\glsentrytext{bec})}
}
\newglossaryentry{awgn}
{
  name={AWGN},
  description={additive white Gaussian noise},
  first={\glsentrydesc{awgn} (\glsentrytext{awgn})}
}
\newglossaryentry{3gpp}
{
  name={3GPP},
  description={3rd generation partnership project},
  first={\glsentrydesc{3gpp} (\glsentrytext{3gpp})}
}

\newglossaryentry{dl}
{
  name={DL},
  description={downlink},
  first={\glsentrydesc{dl} (\glsentrytext{dl})}
}

\newglossaryentry{LED}
{
  name={LED},
  description={light emitting diode},
  first={\glsentrydesc{LED} (\glsentrytext{LED})},
  plural={LEDs},
  descriptionplural={light emitting diodes},
  firstplural={\glsentrydescplural{LED} (\glsentryplural{LED})}
}

\newglossaryentry{lte}
{
  name={LTE},
  description={long term evolution},
  first={\glsentrydesc{lte} (\glsentrytext{lte})}
}
\newglossaryentry{ofdm}
{
  name={OFDM},
  description={orthogonal frequency-division multiplexing},
  first={\glsentrydesc{ofdm} (\glsentrytext{ofdm})}
}

\newglossaryentry{ul}
{
  name={UL},
  description={uplink},
  first={\glsentrydesc{ul} (\glsentrytext{ul})}
}
\newglossaryentry{rb}
{
  name={RB},
  description={resource block},
  first={\glsentrydesc{rb} (\glsentrytext{rb})},
  plural={RBs},
  descriptionplural={resource blocks},
  firstplural={\glsentrydescplural{rb} (\glsentryplural{rb})}
}
\newglossaryentry{cu}
{
  name={CU},
  description={channel use},
  first={\glsentrydesc{cu} (\glsentrytext{cu})},
  plural={CUs},
  descriptionplural={channel uses},
  firstplural={\glsentrydescplural{cu} (\glsentryplural{cu})}
}
\newglossaryentry{tti}
{
  name={TTI},
  description={transmission time interval},
  first={\glsentrydesc{tti} (\glsentrytext{tti})},
  plural={TTI's},
  descriptionplural={transmission time intervals},
  firstplural={\glsentrydescplural{tti} (\glsentryplural{tti})}
}
\newglossaryentry{iid}
{
  name={i.i.d.},
  description={independent and identically distributed},
  first={\glsentrydesc{iid} (\glsentrytext{iid})}
}
\newglossaryentry{psd}
{
  name={PSD},
  description={power spectral density},
  first={\glsentrydesc{psd} (\glsentrytext{psd})}
}

\newglossaryentry{mimo}
{
  name={MIMO},
  description={multiple-input multiple-output},
  first={\glsentrydesc{mimo} (\glsentrytext{mimo})}
}

\newglossaryentry{bler}
{
  name={BLER},
  description={block error probability},
  first={\glsentrydesc{bler} (\glsentrytext{bler})}
}
\newglossaryentry{mtc}
{
  name={MTC},
  description={machine-type communication},
  first={\glsentrydesc{mtc} (\glsentrytext{mtc})}
}
% \newglossaryentry{csi}
% {
%   name=CSI,
%   description={c{hannel state information}},
%   first={\glsentrydesc{csi} (\glsentrytext{csi})}
% }
\newacronym{csi}{CSI}{channel state information}
\newglossaryentry{dvbt}
{
  name={DVB-T},
  description={terrestrial digital video broadcasting},
  first={\glsentrydesc{dvbt} (\glsentrytext{dvbt})}
}
\newglossaryentry{pat}
{
  name={PAT},
  description={pilot-assisted transmission},
  first={\glsentrydesc{pat} (\glsentrytext{pat})}
}
\newglossaryentry{ml}
{
  name={ML},
  description={maximum likelihood},
  first={\glsentrydesc{ml} (\glsentrytext{ml})}
}
\newglossaryentry{dt}
{
  name={DT},
  description={dependence-testing},
  first={\glsentrydesc{dt} (\glsentrytext{dt})}
}
\newglossaryentry{ustm}
{
  name={USTM},
  description={unitary space-time modulation},
  first={\glsentrydesc{ustm} (\glsentrytext{ustm})}
}
\newglossaryentry{siso}
{
  name={SISO},
  description={single-input single-output},
  first={\glsentrydesc{siso} (\glsentrytext{siso})}
}
\newglossaryentry{snn}
{
  name={SNN},
  description={scaled nearest-neighbor},
  first={\glsentrydesc{snn} (\glsentrytext{snn})}
}

\newglossaryentry{snnd}
{
  name={SNND},
  description={scaled nearest-neighbor decoding},
  first={\glsentrydesc{snnd} (\glsentrytext{snnd})}
}
\newglossaryentry{rcus}
{
  name={RCUs},
  description={random-coding union bound with parameter $s$},
  first={\glsentrydesc{rcus} (\glsentrytext{rcus})}
}
\newglossaryentry{osd}
{
  name={OSD},
  description={ordered statistics decoding},
  first={\glsentrydesc{osd} (\glsentrytext{osd})}
}
\newglossaryentry{llr}
{
  name={LLR},
  description={log-likelihood ratio},
  first={\glsentrydesc{llr} (\glsentrytext{llr})}
   plural={LLR's},
  descriptionplural={log-likelihood ratios},
  firstplural={\glsentrydescplural{llr} (\glsentryplural{llr})}
}
\newglossaryentry{qpsk}
{
  name={QPSK},
  description={quaternary phase shift keying},
  first={\glsentrydesc{qpsk} (\glsentrytext{qpsk})}
}
\newglossaryentry{nlos}
{
  name={NLOS},
  description={non-line-of-sight},
  first={\glsentrydesc{nlos} (\glsentrytext{nlos})}
}
\newglossaryentry{los}
{
  name={LOS},
  description={line-of-sight},
  first={\glsentrydesc{los} (\glsentrytext{los})}
}
\newglossaryentry{mgf}
{
  name={MGF},
  description={moment-generating function},
  first={\glsentrydesc{mgf} (\glsentrytext{mgf})}
}
\newglossaryentry{cgf}
{
  name={CGF},
  description={cumulant-generating function},
  first={\glsentrydesc{cgf} (\glsentrytext{cgf})},
  plural={CGFs},
  descriptionplural={cumulant-generating functions},
  firstplural={\glsentrydescplural{cgf} (\glsentryplural{cgf})}
}
\newglossaryentry{pdf}
{
  name={PDF},
  description={probability density function},
  first={\glsentrydesc{pdf} (\glsentrytext{pdf})},
   plural={PDF's},
  descriptionplural={probability density functions},
  firstplural={\glsentrydescplural{pdf} (\glsentryplural{pdf})}
}

\newglossaryentry{ccdf}
{
  name={CCDF},
  description={complementary cumulative distribution function},
  first={\glsentrydesc{ccdf} (\glsentrytext{ccdf})}
}

\newglossaryentry{cdf}
{
  name={CDF},
  description={cumulative distribution function},
  first={\glsentrydesc{cdf} (\glsentrytext{cdf})}
}

\newglossaryentry{gmi}
{
  name={GMI},
  description={generalized mutual information},
  first={\glsentrydesc{gmi} (\glsentrytext{gmi})}
}

\newglossaryentry{arq}
{
  name={ARQ},
  description={automatic repeat request},
  first={\glsentrydesc{arq} (\glsentrytext{arq})}
}

\newglossaryentry{harq}
{
  name={HARQ},
  description={hybrid automatic repeat request},
  first={\glsentrydesc{harq} (\glsentrytext{harq})}
}

\newglossaryentry{fbl}
{
  name={FBL-NF},
  description={fixed blocklength with no feedback},
  first={\glsentrydesc{fbl} (\glsentrytext{fbl})}
}
\newglossaryentry{ssnf}
{
  name={SS-NF},
  description={single-shot no-feedback},
  first={\glsentrydesc{ssnf} (\glsentrytext{ssnf})}
}

% \newglossaryentry{urllc}
% {
%   name={URLLC},
%   description={ultra-reliable low-latency communications},
%   first={\glsentrydesc{urllc} (\glsentrytext{urllc})}
% }
\newacronym{urllc}{URLLC}{ultra-reliable low-latency communications}

\newglossaryentry{vlsf}
{
  name={VLSF},
  description={Variable-length stop-feedback},
  first={\glsentrydesc{vlsf} (\glsentrytext{vlsf})}
}

\newglossaryentry{vlnsf}
{
  name={VLNSF},
  description={variable-length noisy stop feedback},
  first={\glsentrydesc{vlnsf} (\glsentrytext{vlnsf})}
}

\newglossaryentry{dmt}
{
  name={DMT},
  description={diversity-multiplexing tradeoff},
  first={\glsentrydesc{dmt} (\glsentrytext{dmt})}
}

\newglossaryentry{dmdt}
{
  name={DMDT},
  description={diversity-multiplexing-delay tradeoff},
  first={\glsentrydesc{dmdt} (\glsentrytext{dmdt})}
}

\newglossaryentry{tddt}
{
  name={TDDT},
  description={throughput-diversity-delay tradeoff},
  first={\glsentrydesc{tddt} (\glsentrytext{tddt})}
}

\newglossaryentry{tdd}
{
  name={TDD},
  description={time-division duplex},
  first={\glsentrydesc{tdd} (\glsentrytext{tdd})}
}

\newglossaryentry{stbc}
{
  name={STBC},
  description={space-time block-codes},
  first={\glsentrydesc{stbc} (\glsentrytext{stbc})},
  plural={STBC's},
  descriptionplural={space-time block-codes},
  firstplural={\glsentrydescplural{stbc} (\glsentryplural{stbc})}
}

\newglossaryentry{harqir}
{
  name={HARQ-IR},
  description={hybrid automatic repeat request with incremental redundancy},
  first={\glsentrydesc{harqir} (\glsentrytext{harqir})}
}

\newglossaryentry{harqcc}
{
  name={HARQ-CC},
  description={hybrid automatic repeat request with chase combining},
  first={\glsentrydesc{harqcc} (\glsentrytext{harqcc})}
}

\newglossaryentry{wp1}
{
  name={w.p.1.},
  description={with probability one},
  first={\glsentrydesc{wp1} (\glsentrytext{wp1})}
}

\newglossaryentry{vlff}
{
  name={VLFF},
  description={variable-length full feedback},
  first={\glsentrydesc{vlff} (\glsentrytext{vlff})}
}

\newglossaryentry{dmc}
{
  name={DMC},
  description={discrete memoryless channel},
  first={\glsentrydesc{dmc} (\glsentrytext{dmc})}
  plural={DMCs},
  descriptionplural={discrete memoryless channels},
  firstplural={\glsentrydescplural{dmc} (\glsentryplural{dmc})}
}



==> fig/patterntikz.tex <==
\usepackage{tikz}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes,arrows,positioning}
\usetikzlibrary{calc}
\usetikzlibrary{fit}
\usetikzlibrary{plotmarks}
\tikzset{every picture/.style={font issue=\scriptsize, >=stealth},font issue/.style={execute at begin picture={#1\selectfont}}}
\tikzset{three sided left/.style={
        draw=none,
        xshift=\pgflinewidth,
        append after command={
            [shorten <= -0.5\pgflinewidth]
            ([shift={(-1.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north east) edge ([shift={( 0.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north west) 
            ([shift={( 0.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north west) edge ([shift={( 0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south west)            
            ([shift={( 0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south west) edge ([shift={(-1.0\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south east)
        }}}
        
\tikzset{three sided right/.style={
        draw=none,
        xshift=-\pgflinewidth,
        append after command={
            [shorten <= -0.5\pgflinewidth]
            ([shift={( 1.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north west) edge ([shift={(-0.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north east) 
            ([shift={(-0.5\pgflinewidth,-0.5\pgflinewidth)}]\tikzlastnode.north east) edge ([shift={(-0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south east)            
            ([shift={(-0.5\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south east) edge ([shift={( 1.0\pgflinewidth,+0.5\pgflinewidth)}]\tikzlastnode.south west)
        }}}
        
\newcommand{\drawdimline}[2]{\draw [|<->|] ($(#1)+(-0.5\pgflinewidth,0)$)--($(#2) + (0.5\pgflinewidth,0)$)}        
        
%\newcommand\dimarr[3][]{ \draw[dimarr, |<->|] (#1) -- (#2) node[midway,below]{#3}; }  

\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}
\pgfplotsset{
  compat=newest, % Allows drawing of circles.
  width=\columnwidth,    %0.86\columnwidth,  
  height=0.8\columnwidth,   %0.60\columnwidth, 
  plot coordinates/math parser=false,
  standard/.style={
    axis equal,
    axis line style=help lines,
    axis x line=center,
    axis y line=center,
    axis z line=center},
    grid style={dashed,gray},
    minor grid style={dotted,gray},
    major grid style={dotted,gray},
    ylabel absolute, ylabel style={yshift=-0.4cm},
    xlabel absolute, xlabel style={yshift=0.25cm}
}

\makeatletter
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\LineWidth]{my horizontal lines}%
    {\pgfpointorigin}{\pgfqpoint{100pt}{1pt}}{\pgfqpoint{100pt}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{0pt}{0.5pt}}
        \pgfpathlineto{\pgfqpoint{100pt}{0.5pt}}
        \pgfusepath{stroke}
    }
 
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\LineWidth]{my vertical lines}%
    {\pgfpointorigin}{\pgfqpoint{1pt}{100pt}}{\pgfqpoint{\LineSpace}{100pt}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{0.5pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{0.5pt}{100pt}}
        \pgfusepath{stroke}
    } 
 
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\LineWidth]{my grid}%
    {\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{0pt}{\LineSpace + 0.1pt}}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{0pt}}
        \pgfusepath{stroke}
    }
 
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\LineWidth]{my north east lines}
    {\pgfqpoint{-\LineWidth}{-\LineWidth}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{-\LineWidth}{-\LineWidth}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{\LineSpace + 0.1pt}}
        \pgfusepath{stroke}
    }
 
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\LineWidth]{my north west lines}
    {\pgfqpoint{-\LineWidth}{-\LineWidth}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{-\LineWidth}{\LineSpace}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{-\LineWidth}}
        \pgfusepath{stroke}
    }
 
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\LineWidth]{my crosshatch}%
    {\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{\LineSpace}{\LineSpace}}
    {\pgfqpoint{\LineSpace}{\LineSpace}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\LineWidth}
        \pgfpathmoveto{\pgfqpoint{\LineSpace + 0.1pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{0pt}{\LineSpace + 0.1pt}}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{\LineSpace + 0.1pt}{\LineSpace + 0.1pt}}
        \pgfusepath{stroke}
    }
 
 \pgfdeclarepatternformonly[\tikz@pattern@color,\LineSpace,\PointSize]{my dots}%
    {\pgfqpoint{-\LineSpace*0.25}{-\LineSpace*0.25}}
    {\pgfqpoint{\LineSpace*0.25}{\LineSpace*0.25}}
    {\pgfqpoint{\LineSpace*0.75}{\LineSpace*0.75}}%
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{\PointSize}
        \pgfusepath{fill}
    }
\makeatother
 
\newdimen\LineSpace
\newdimen\PointSize
\newdimen\LineWidth
\tikzset{
    line space/.code={\LineSpace=#1},
    line space=3pt
}
\tikzset{
    point size/.code={\PointSize=#1},
    point size=.5pt
}
\tikzset{
    pattern line width/.code={\LineWidth=#1},
    pattern line width=.4pt
}

% Add nodes on the curves drawn using pfgplots \addplot
% Add a node inside the axis at a given axis coordinate
% \node[name=lin_graph_point] at (axis cs:11,0.0245){};
% Add a node along the plotted path at 0.75 from the start point
%\addplot[][]{} coordinate[pos=0.75](lin_graph_point);

  


==> fig/symbols.tex <==


\newcommand{\defeq}{\mathrel{\mkern-0.25mu=}}
%\newcommand{\safemath}[2]{\newcommand{#1}{\ensuremath{#2}\xspace}}
\DeclareSymbolFontAlphabet{\amsmathbb}{AMSb}%

%\newcommand{\lefto}{\mathopen{}\left}
%---------------------------------------------------------------------------------------------------------------------------------------------------------------
%																	Miscellaneous
%---------------------------------------------------------------------------------------------------------------------------------------------------------------
\newcommand{\lro}[1]{\lefto({#1}\right)}																% left right paranthesis operator
\newcommand{\lrbo}[1]{\lefto \lbrace {#1} \right \rbrace}															% left right braces operator
\newcommand{\lrho}[1]{\lefto [ {#1} \right ]}																				% left right hard braces operator

\newcommand{\lr}[1]{\left({#1}\right)}																% left right paranthesis operator
\newcommand{\lrb}[1]{\left \lbrace {#1} \right \rbrace}															% left right braces operator
\newcommand{\lrh}[1]{\left [ {#1} \right ]}																				% left right hard braces operator


%---------------------------------------------------------------------------------------------------------------------------------------------------------------
%																	Wireless communication
%---------------------------------------------------------------------------------------------------------------------------------------------------------------
\safemath{\dopplerspread}{B_D}																								% doppler spread
\safemath{\delayspread}{T_D}																									% delay spread
\safemath{\nc}{n\sub{c}}																										% coherence time
\safemath{\nf}{n\sub{f}}																										% feedback message length
\safemath{\efa}{p\sub{sc}}
\safemath{\efb}{p\sub{cs}}
\safemath{\ef}{\epsilon\sub{f}	}
\safemath{\nd}{n\sub{d}}																										% data symbols
\safemath{\ntx}{n\sub{t}} 																											% transmit antennas
\safemath{\nrx}{n\sub{r}}																											% receive antennas
\safemath{\ntxt}{\tilde{n\sub{t}}}																											% receive antennas
\safemath{\cb}{\ensuremath{L}} 																								% code blocks
\safemath{\cl}{\ensuremath{n}} 																								% codelength
\safemath{\txanto}{{\ensuremath{\tilde{m}_t}}} 																		% transmit antennas when some is turned off
\safemath{\cs}{M} 																														% code size
\safemath{\idPustm}{\ensuremath{S_{k}}}
\safemath{\error}{\ensuremath{\epsilon}} 																				%Error target
\safemath{\eexp}{\ensuremath{\mathcal{E}}} 																			%Error exponent
\safemath{\nsubc}{n\sub{s}}			 																						% number of subcarriers
\safemath{\nofdm}{n\sub{o}} 																									% number of OFDM symbols
\safemath{\bc}{\ensuremath{B_c}} 																							% Coherence bandwidth
\safemath{\ts}{\ensuremath{T_s}} 																							% Symbol time
\safemath{\nrb}{\ensuremath{n_{rb}}} 																						% Symbol time
\safemath{\rul}{\ensuremath{\rho\sub{ul}}}
\safemath{\rdl}{\ensuremath{\rho\sub{dl}}}

\safemath{\nres}{\ell}
\safemath{\nr}{n\sub{r}}
\newcommand{\cgauss}[2]{\mathcal{CN}\lro{\ensuremath{#1, #2}  }}   								% complex gaussian
\safemath{\maxk}{M^*\lr{\nres, \nsubc, \nofdm, \epsilon, \rho}}
\safemath{\Rmax}{R^*}%\lr{\nres, \nsubc, \nofdm,M, \epsilon, \rho}}
\safemath{\Emin}{E\sub{b}^*/N_0}%\lr{\nres, \nsubc, \nofdm,M, \epsilon, \rho}}
\safemath{\Eminf}{\frac{E\sub{b}^*}{N_0}}
\safemath{\np}{\ensuremath{n\sub{p}}}
\safemath{\ndf}{\ensuremath{\bar{n}\sub{d}}}
\safemath{\npf}{\ensuremath{\bar{n}\sub{p}}}
\safemath{\code}{\ensuremath{\mathcal{C}}}
\safemath{\err}{\ensuremath{\epsilon}}
\safemath{\rp}{\ensuremath{\rho\sub{p}}}
\safemath{\rd}{\ensuremath{\rho\sub{d}}}
\safemath{\cohtime}{\ensuremath{T\sub{c}}}
\safemath{\cohbw}{\ensuremath{B\sub{c}}}
\safemath{\nmax}{\ensuremath{\ell\sub{m}}}
\safemath{\ntot}{\ensuremath{n\sub{tot}}}
\safemath{\nul}{\ensuremath{n\sub{ul}}}
\safemath{\ndl}{\ensuremath{n\sub{dl}}}

\safemath{\yp}{\ensuremath{\randvecy_{\nu}^{(\text{p})}}}
\safemath{\yd}{\ensuremath{\randvecy_{\nu}^{(\text{d})}}}
\safemath{\ypd}{\ensuremath{\vecy_{\nu}^{(\text{p})}}}
\safemath{\ydd}{\ensuremath{\vecy_{\nu}^{(\text{d})}}}

\safemath{\ypf}{\ensuremath{\bar{\randvecy}_{\nu}^{(\text{p})}}}
\safemath{\ydf}{\ensuremath{\bar{\randvecy}_{\nu}^{(\text{d})}}}
\safemath{\ypdf}{\ensuremath{\bar{\vecy}_{\nu}^{(\text{p})}}}
\safemath{\yddf}{\ensuremath{\bar{\vecy}_{\nu}^{(\text{d})}}}

\safemath{\xp}{\ensuremath{\vecx^{(\text{p})}}}
\safemath{\xd}{\ensuremath{\randvecx_{\nu}^{(\text{d})}}}
\safemath{\xdd}{\ensuremath{\vecx_{\nu}^{(\text{d})}}}

\safemath{\xpf}{\ensuremath{\bar{\vecx}^{(\text{p})}}}
\safemath{\xdf}{\ensuremath{\bar{\randvecx}_{\nu}^{(\text{d})}}}
\safemath{\xddf}{\ensuremath{\bar{\vecx}_{\nu}^{(\text{d})}}}

\safemath{\xdb}{\ensuremath{\overline{\randvecx}^{(\text{d})}}}
\safemath{\Pxd}{\ensuremath{P_{\randvecx^{(\text{d})}}}}


\safemath{\xpbar}{\ensuremath{\overline{\matX}^{(\text{p})}}}
\safemath{\xdbar}{\ensuremath{\overline{\randmatX}^{(\text{d})}}}

\safemath{\xdv}{\ensuremath{\randvecx^{(\text{d})}}}
\safemath{\xdbarv}{\ensuremath{\overline{\randvecx}^{(\text{d})}}}
\safemath{\ydv}{\ensuremath{\randvecy^{(\text{d})}}}

\safemath{\xdr}{\ensuremath{\matX^{(\text{d})}}}

\safemath{\ttx}{\ensuremath{\tau\sub{tx}}}
\safemath{\trx}{\ensuremath{\tau\sub{rx}}}
\safemath{\ack}{\ensuremath{\mathrm{s}}}
\safemath{\nack}{\ensuremath{\mathrm{c}}}

\newcommand{\prob}[1]{\ensuremath{\mathbb{P}\lrho{#1}}}


%---------------------------------------------------------------------------------------------------------------------------------------------------------------
%																	Information theory
%---------------------------------------------------------------------------------------------------------------------------------------------------------------
\safemath{\mI}{\ensuremath{i\lro{\randvecy ; \randvecx}}} 				% i(Y;X)
\newcommand{\mIs}[1]{i\lro{\randvecy_{#1} ; \randvecx_{#1}}}		% i(Y_l;X_l)
\newcommand{\mmi}[1]{q\lro{\randvecy ; #1}}						% i(Y;x(m))
\newcommand{\mmib}[1]{q\lro{\bar{\randvecy} ; #1}}						% i(Y;x(m))
\newcommand{\thres}[1]{\gamma\lro{#1}}						% i(Y;x(m))


%---------------------------------------------------------------------------------------------------------------------------------------------------------------
%																	Math operators
%---------------------------------------------------------------------------------------------------------------------------------------------------------------


\safemath{\randveca}{\bm{A}}
\safemath{\randvecb}{\bm{B}}
\safemath{\randvecc}{\bm{C}}
\safemath{\randvecd}{\bm{D}}
\safemath{\randvece}{\bm{E}}
\safemath{\randvecf}{\bm{F}}
\safemath{\randvecg}{\bm{G}}
\safemath{\randvech}{\bm{H}}
\safemath{\randveci}{\bm{I}}
\safemath{\randvecj}{\bm{J}}
\safemath{\randveck}{\bm{K}}
\safemath{\randvecl}{\bm{L}}
\safemath{\randvecm}{\bm{M}}
\safemath{\randvecn}{\bm{N}}
\safemath{\randveco}{\bm{O}}
\safemath{\randvecp}{\bm{P}}
\safemath{\randvecq}{\bm{Q}}
\safemath{\randvecr}{\bm{R}}
\safemath{\randvecs}{\bm{S}}
\safemath{\randvect}{\bm{T}}
\safemath{\randvecu}{\bm{U}}
\safemath{\randvecv}{\bm{V}}
\safemath{\randvecw}{\bm{W}}
\safemath{\randvecx}{\bm{X}}
\safemath{\randvecy}{\bm{Y}}
\safemath{\randvecz}{\bm{Z}}
\safemath{\randvecphi}{\bm{\Phi}}


\safemath{\randmatA}{\amsmathbb{A}}
\safemath{\randmatB}{\amsmathbb{B}}
\safemath{\randmatC}{\amsmathbb{C}}
\safemath{\randmatD}{\amsmathbb{D}}
\safemath{\randmatE}{\amsmathbb{E}}
\safemath{\randmatF}{\amsmathbb{F}}
\safemath{\randmatG}{\amsmathbb{G}}
\safemath{\randmatH}{\amsmathbb{H}}
\safemath{\randmatI}{\amsmathbb{I}}
\safemath{\randmatJ}{\amsmathbb{J}}
\safemath{\randmatK}{\amsmathbb{K}}
\safemath{\randmatL}{\amsmathbb{L}}
\safemath{\randmatM}{\amsmathbb{M}}
\safemath{\randmatN}{\amsmathbb{N}}
\safemath{\randmatO}{\amsmathbb{O}}
\safemath{\randmatP}{\amsmathbb{P}}
\safemath{\randmatQ}{\amsmathbb{Q}}
\safemath{\randmatR}{\amsmathbb{R}}
\safemath{\randmatS}{\amsmathbb{S}}
\safemath{\randmatT}{\amsmathbb{T}}
\safemath{\randmatU}{\amsmathbb{U}}
\safemath{\randmatV}{\amsmathbb{V}}
\safemath{\randmatW}{\amsmathbb{W}}
\safemath{\randmatX}{\amsmathbb{X}}
\safemath{\randmatY}{\amsmathbb{Y}}
\safemath{\randmatZ}{\amsmathbb{Z}}
\safemath{\randmatSigma}{\mathbb{\Sigma}}
\safemath{\randmatPhi}{\mathbb{\Phi}}
\safemath{\randmatLambda}{\mathbb{\Lambda}}



\safemath{\matSigma}{\bm{\Sigma}}
\safemath{\matPhi}{\bm{\Phi}}
\safemath{\matLambda}{\bm{\Lambda}}

